Local Aggregation for Unsupervised Learning of Visual Embeddings

Unsupervised approaches to learning in neural networks are of substantial interest for furthering artificial intelligence, both because they would enable the training of networks without the need for large numbers of expensive annotations, and because they would be better models of the kind of general-purpose learning deployed by humans. However, unsupervised networks have long lagged behind the performance of their supervised counterparts, especially in the domain of large-scale visual recognition. Recent developments in training deep convolutional embeddings to maximize non-parametric instance separation and clustering objectives have shown promise in closing this gap. Here, we describe a method that trains an embedding function to maximize a metric of local aggregation, causing similar data instances to move together in the embedding space, while allowing dissimilar instances to separate. This aggregation metric is dynamic, allowing soft clusters of different scales to emerge. We evaluate our procedure on several large-scale visual recognition datasets, achieving state-of-the-art unsupervised transfer learning performance on object recognition in ImageNet, scene recognition in Places 205, and object detection in PASCAL VOC.

==> latex/sections/tables/kmeans_combine.tex <==
\begin{table}
\begin{center}
\begin{tabular}{c|ccc}
\hline
\diagbox[width=7em]{Setting}{Network} & AlexNet & ResNet-18 & ResNet-50 \\
\hline\hline
\\[-1em]
$\bigcap^3 \mathrm{KM}_{10000}$ & -- & 34.3 & -- \\ 
\hline
$\mathrm{KM}_{1000}$ & -- & 35.2 & -- \\
\hline
$\mathrm{KM}_{10000}$ & 30.6 & 35.7 & 40.2 \\
\hline
$\mathrm{KM}_{20000}$ & -- & 35.0 & -- \\
\hline
\\[-1em]
$\bigcup^3 \mathrm{KM}_{10000}$ & \textbf{31.1} & 36.2 & --\\
\hline
\\[-1em]
$\bigcup^6 \mathrm{KM}_{10000}$ & 30.4 & 37.3 & 42.4 \\
\hline
\\[-1em]
$\bigcup^{10} \mathrm{KM}_{10000}$ & -- & 36.2 & 42.3 \\
\hline
\\[-1em]
$\bigcup^{10} \mathrm{KM}_{30000}$ & -- & \textbf{37.9} & \textbf{43.4} \\
\hline
\end{tabular}
\end{center}
\caption{
Best validation performances in percentages for networks trained with different combination operations and parameters.
Numbers in bold are the best performances in columns.
}
\label{tab:combine}
\end{table}

==> latex/sections/tables/neighbor_table.tex <==
\begin{table}
\begin{center}
\begin{tabular}{c|c|c|c}
\hline
\diagbox[width=5em]{$\SemNei$}{$\ConNei$} & \thead{Nearest: \\ $\mathcal{N}_{4096}$} & \thead{Clustering: \\ $\mathrm{KM}_{300}$} & $U$ \\
\hline\hline
$\{i\}$ & 33.9 & ?? & ??  \\
\hline
\thead{Nearest: \\ $\mathcal{N}_{\{2, 5, 10, 20, 100, 200\}}$} & \texttt{NT} & \texttt{NT} & \texttt{NT}  \\
\hline
\thead{Clustering: \\ $\mathrm{KM}_{10000}$} & \textbf{35.7} & 33.2 & 30.2  \\
\hline
\end{tabular}
\end{center}
\caption{
Best validation performances in percentages for networks trained with different neighbor identification procedures for semantic and context neighbors.
\texttt{NT} means the model is \textbf{NOT} trainable under that setting.
$U$ represents $\{1, 2, ..., N\}$.
$\mathrm{KM}_k$ means the clustering results by KMeans algorithm with $k$ clusters.
}
\label{tab:nei}
\end{table}

==> latex/sections/tables/place_table_back.tex <==
\begin{table}
\begin{center}
\begin{tabular}{c|ccccc|c}
\hline
Method & conv1 & conv2 & conv3 & conv4 & conv5 & KNN \\
\hline\hline
\multicolumn{7}{c}{AlexNet}\\
\hline
Random & 15.7 & 20.3 & 19.8 & 19.1 & 17.5 & 3.9 \\
Data-Init~\cite{krahenbuhl2015data} & 21.4 & 26.2 & 27.1 & 26.1 & 24.0 & -- \\
Context~\cite{doersch2015unsupervised} & 19.7 & 26.7 & 31.9 & 32.7 & 30.9 & -- \\
Adversarial~\cite{donahue2016adversarial} & 17.7 & 24.5 & 31.0 & 29.9 & 28.0 & -- \\
Video~\cite{wang2015unsupervised} & 22.0 & 28.7 & 31.8 & 31.3 & 29.7 & -- \\
Color~\cite{zhang2016colorful} & 22.0 & 28.7 & 31.8 & 31.3 & 29.7 & -- \\
Jigsaw~\cite{noroozi2016unsupervised} & \textbf{23.0} & 32.1 & 35.5 & 34.8 & 31.3 & -- \\
SplitBrain~\cite{zhang2017split} & 21.3 & 30.7 & 34.0 & 34.1 & 32.5 & 10.8 \\
IR~\cite{wu2018unsupervised} & 18.8 & 24.3 & 31.9 & 34.5 & 33.6 & 30.1 \\
IR(with BN)* & 21.3 & 33.0 & 36.5 & 39.2 & 38.7 & ?? \\
DC~\cite{caron2018deep} & 19.6 & \textbf{33.2} & \textbf{39.2} & 39.8 & 34.7 & -- \\
Ours & 18.7 & 32.7 & 38.2 & \fcolorbox{red}{white}{\textbf{40.3}} & \textbf{39.5} & ?? \\
\hline
\multicolumn{7}{c}{VGG16}\\
\hline
IR & 17.6 & 23.1 & 29.5 & 33.8 & 36.3 & 32.8 \\
IR(with BN)* & 18.3 & 23.9 & 30.1 & 41.6 & 45.1 & ?? \\
DC* & \textbf{21.5} & \textbf{31.6} & \textbf{40.9} & \textbf{45.2}  & 44.2  & --   \\
Ours$\dagger$ & 19.1 & 24.9 & 31.3 & 43.4 & \fcolorbox{red}{white}{\textbf{49.3}} & ?? \\
\hline
\multicolumn{7}{c}{ResNet-18}\\
\hline
IR & 17.8 & 23.0 & 30.1 & 37.0 & 38.1 & 38.6 \\
DC* & 16.4 & 22.5 & 30.5 & 40.4 & 41.8 & --  \\
Ours & \textbf{18.9} & \textbf{26.7} & \textbf{36.5} & \textbf{44.7} & \fcolorbox{red}{white}{\textbf{45.6}} & ?? \\
\hline
\multicolumn{7}{c}{ResNet-50}\\
\hline
IR & 18.1 & 22.3 & 29.7 & 42.1 & 45.5 & 41.6 \\
DC* & \textbf{20.1} & \textbf{29.1}  & 35.3 & 43.2 & 38.9  & --   \\
Ours & 10.3 & 26.4 & \textbf{39.9} & \textbf{47.2} & \fcolorbox{red}{white}{\textbf{50.1}} & ?? \\
\hline
\end{tabular}
\end{center}
\caption{
Places transfer learning and KNN classifier performances.
Bold numbers are the best in their columns compared to other tasks using the same architecture.
Most performances are taken from~\cite{caron2018deep, wu2018unsupervised}.
*: performances produced by us, please refer to the supplementary material for more information. 
$\dagger$: our VGG16 is one layer shallower than standard VGG16, see the supplementary material.
}
\label{tab:places}
\end{table}
